ISPY: Automatic Issue-Solution Pair Extraction from Community Live Chats

Collaborative live chats are gaining popularity as a development communication tool. In community live chatting, developers are likely to post issues they encountered (e.g., setup issues and compile issues), and other developers respond with possible solutions. Therefore, community live chats contain rich sets of information for reported issues and their corresponding solutions, which can be quite useful for knowledge sharing and future reuse if extracted and restored in time. However, it remains challenging to accurately mine such knowledge due to the noisy nature of interleaved dialogs in live chat data. In this paper, we first formulate the problem of issue-solution pair extraction from developer live chat data, and propose an automated approach, named ISPY, based on natural language processing and deep learning techniques with customized enhancements, to address the problem. Specifically, ISPY automates three tasks: 1) Disentangle live chat logs, employing a feedforward neural network to disentangle a conversation history into separate dialogs automatically; 2) Detect dialogs discussing issues, using a novel convolutional neural network (CNN), which consists of a BERT-based utterance embedding layer, a context-aware dialog embedding layer, and an output layer; 3) Extract appropriate utterances and combine them as corresponding solutions, based on the same CNN structure but with different feeding inputs. To evaluate ISPY, we compare it with six baselines, utilizing a dataset with 750 dialogs including 171 issue-solution pairs and evaluate ISPY from eight open source communities. The results show that, for issue-detection, our approach achieves the F1 of 76%, and outperforms all baselines by 30%. Our approach achieves the F1 of 63% for solution-extraction and outperforms the baselines by 20%.

==> tab/ablation.tex <==
\begin{table*}[htbp]
\centering
 \resizebox{\textwidth}{!}{
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|}
\hline
\multirow{2}{*}{\textbf{Task}} & \multirow{2}{*}{\textbf{Methods}} & \multicolumn{3}{c|}{\textbf{Angular}} & \multicolumn{3}{c|}{\textbf{Appium}} & \multicolumn{3}{c|}{\textbf{Docker}} & \multicolumn{3}{c|}{\textbf{DL4j}} & \multicolumn{3}{c|}{\textbf{Ethereum}} & \multicolumn{3}{c|}{\textbf{Gitter}} & \multicolumn{3}{c|}{\textbf{Nodejs}} & \multicolumn{3}{c|}{\textbf{Typescript}} &
\multicolumn{3}{c|}{\textbf{Average}}\\
\cline{3-29}
& & P & R & F1 & P & R & F1 & P & R & F1 & P & R & F1 & P & R & F1 & P & R & F1 & P & R & F1 & P & R & F1 & P & R & F1  \\
\hline
\multirow{7}{*}{Issue} & RICHA & \cellcolor{pink}0.76 & \cellcolor{pink}0.77 & \cellcolor{pink}0.76 & \cellcolor{pink}0.75 & 0.68 & \cellcolor{pink}0.71 & \cellcolor{pink}0.84 & 0.74 & \cellcolor{pink}0.79 & 0.77 & \cellcolor{pink}0.68 & \cellcolor{pink}0.72 & 0.82 & 0.73 & \cellcolor{pink}0.77 & \cellcolor{pink}0.80 & \cellcolor{pink}0.69 & \cellcolor{pink}0.74 & \cellcolor{pink}0.79 & 0.70 & \cellcolor{pink}0.74 & \cellcolor{pink}0.86 & \cellcolor{pink}0.78 & \cellcolor{pink}0.82 & \cellcolor{orange}0.80 & \cellcolor{orange}0.72 & \cellcolor{orange}0.76\\
\cline{2-29} & NB & 0.36 & 0.40 & 0.38 & 0.41 & 0.30 & 0.35 & 0.47 & 0.36 & 0.41 & 0.70 & 0.56 & 0.62 & 0.08 & 0.25 & 0.13 & 0.22 & 0.42 & 0.29 & 0.30 & 0.50 & 0.37 & 0.15 & 0.40 & 0.22 & 0.34 & 0.40 & 0.36 \\
\cline{2-29} & RF & 0.56 & 0.25 & 0.34 & 0.69 & 0.30 & 0.42 & 0.75 & 0.23 & 0.35 & \cellcolor{pink}0.84 & 0.44 & 0.58 & \cellcolor{pink}1.00 & 0.17 & 0.29 & 0.50 & 0.25 & 0.33 & 0.33 & 0.13 & 0.18 & 0.23 & 0.30 & 0.26 & 0.61 & 0.26 & 0.36 \\
\cline{2-29} & GBDT & 0.27 & 0.75 & 0.40 & 0.40 & \cellcolor{pink}0.70 & 0.51 & 0.50 & \cellcolor{pink}0.79 & 0.61 & 0.73 & 0.44 & 0.55 & 0.21 & \cellcolor{pink}0.83 & 0.33 & 0.19 & 0.67 & 0.29 & 0.30 & \cellcolor{pink}0.88 & 0.44 & 0.18 & 0.90 & 0.30 & 0.35 & 0.74 & 0.47 \\
\cline{2-29} & Casper & 0.39 & 0.35 & 0.37 & 0.08 & 0.03 & 0.05 & 0.59 & 0.26 & 0.36 & 0.46 & 0.40 & 0.43 & 0.19 & 0.42 & 0.26 & 0.14 & 0.17 & 0.15 & 0.05 & 0.06 & 0.06 & 0.15 & 0.40 & 0.22 & 0.26 & 0.26 & 0.26 \\
\cline{2-29} & CNC\_PD & 0.20 & 0.55 & 0.29 & 0.23 & 0.50 & 0.32 & 0.23 & 0.36 & 0.28 & 0.12 & 0.32 & 0.17 & 0.24 & 0.42 & 0.30 & 0.12 & 0.42 & 0.19 & 0.10 & 0.50 & 0.17 & 0.05 & 0.40 & 0.10  & 0.16 & 0.43 & 0.24\\
\cline{2-29} & DECA\_PD & 0.33 & 0.50 & 0.40 & 0.28 & 0.37 & 0.31 & 0.33 & 0.36 & 0.34 & 0.64 & 0.28 & 0.39 & 0.42 & 0.42 & 0.42 & 0.44 & 0.67 & 0.53 & 0.32 & 0.50 & 0.39 & 0.04 & 0.10 & 0.06 & 0.35 & 0.40 & 0.37\\
\hline
\multirow{7}{*}{Solution} & RICHA & \cellcolor{pink}0.61 & 0.58 & \cellcolor{pink}0.69 & \cellcolor{pink}0.68 & 0.57 & \cellcolor{pink}0.62 & \cellcolor{pink}0.71 & 0.60 & \cellcolor{pink}0.65 & \cellcolor{pink}0.66 & \cellcolor{pink}0.62 & \cellcolor{pink}0.58 & \cellcolor{pink}0.73 & 0.63 & \cellcolor{pink}0.68 & \cellcolor{pink}0.62 & 0.56 & \cellcolor{pink}0.59 & \cellcolor{pink}0.68 & 0.58 & \cellcolor{pink}0.63 & \cellcolor{pink}0.72 & 0.67 & \cellcolor{pink}0.69 & \cellcolor{orange}0.68 & 0.59 & \cellcolor{orange}0.63\\
\cline{2-29} & NB & 0.21 & 0.58 & 0.30 & 0.24 & 0.48 & 0.32 & 0.31 & 0.59 & 0.40 & 0.58 & 0.49 & 0.53 & 0.33 & \cellcolor{pink}0.80 & 0.47 & 0.10 & \cellcolor{pink}0.67 & 0.17 & 0.37 & 0.55 & 0.44 & 0.08 & 0.09 & 0.09 & 0.28 & 0.53 & 0.37 \\
\cline{2-29} & RF & 0.26 & 0.83 & 0.39 & 0.27 & 0.52 & 0.36 & 0.31 & 0.56 & 0.40 & 0.80 & 0.13 & 0.22 & 0.15 & 0.40 & 0.22 & 0.10 & 0.33 & 0.15 & 0.50 & 0.65 & 0.57 & 0.54 & 0.64 & 0.58 & 0.37 & 0.51 & 0.43 \\
\cline{2-29} & GBDT & 0.26 & \cellcolor{pink}0.92 & 0.40 & 0.26 & \cellcolor{pink}0.74 & 0.38 & 0.22 & \cellcolor{pink}0.62 & 0.32 & 0.71 & 0.16 & 0.26 & 0.11 & 0.40 & 0.17 & 0.10 & 0.67 & 0.17 & 0.42 & \cellcolor{pink}0.75 & 0.54 & 0.42 & \cellcolor{pink}0.73 & 0.53 & 0.31 & \cellcolor{orange}0.62 & 0.41 \\
\cline{2-29} & UIT & 0.29 & 0.17 & 0.21 & 0.21 & 0.13 & 0.17 & 0.30 & 0.12 & 0.17 & 0.24 & 0.07 & 0.12 & 0.37 & 0.16 & 0.22 & 0.27 & 0.11 & 0.17 & 0.19 & 0.15 & 0.18 & 0.31 & 0.18 & 0.23 & 0.27 & 0.14 & 0.18 \\
\cline{2-29} & CNC\_SP & 0.18 & 0.17 & 0.17 & 0.26 & 0.28 & 0.27 & 0.21 & 0.31 & 0.25 & 0.46 & 0.20 & 0.28 & 0.30 & 0.14 & 0.19 & 0.46 & 0.54 & 0.50 & 0.41 & 0.28 & 0.33 & 0.38 & 0.25 & 0.30 & 0.33 & 0.27 & 0.30 \\
\cline{2-29} & DECA\_SP & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.20 & 0.09 & 0.12 & 0.25 & 0.02 & 0.24 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.57 & 0.20 & 0.30 & 0.33 & 0.09 & 0.14 & 0.17 & 0.05 & 0.08 \\
\hline
\end{tabular}}
\caption{Ablation study across eight projects.}
\label{tab:ablation}
\end{table*}

==> tab/badcase.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[htbp]
 \resizebox{\columnwidth}{!}{
\begin{tabular}{|l|}
\hline
\begin{tabular}[c]{@{}l@{}}
{\LARGE \textbf{Raw Dialog}}\\ 
\parbox[c]{12cm}{A(OQ): Good Morning (again!), trying to run arbiter and trying to figure out how to create the DataProvider<DataSetIterator> from RecordReaderDataSetIterator.} \\
B(GG): Go ahead!\\
\parbox[c]{12cm}{A(OQ): Trying [<-CODE->]; but this is not splitting the dataset correctly. \textcolor{red}{How do I create a DataProvider from a RecordReaderDataSetIterator?}}\\
B(IG1): \textcolor{blue}{You'd want to split the data yourself: [<-LINK->].} \\
A(FQ): \textcolor{brown}{Can I use SplitTestAndTrain?}\\
B(IG2.1): Not really, unless you have the whole dataset in memory.\\
B(IG2.2): You could go through the iterator and randomly do split test train and save the results.\\
A(NF): I tried [<-CODE->] Does this not work?\\
B(IG3.1): \textcolor{purple}{You could do split test and train on the batches and concatenate.}\\
\parbox[c]{12cm}{B(IG3.2): \textcolor{purple}{My batchsize is the entire dataset so should be fine, then split test and train will work.}}\\
A(PF): Many thanks.
\end{tabular}\\
\hline

\begin{tabular}[c]{@{}l@{}}
{\LARGE \textbf{Ground Truth}}\\ 
\textit{Basic issue}: \textcolor{red}{How do I create a DataProvider from a RecordReaderDataSetIterator?}\\
\textit{Solution for basic issue}: \textcolor{blue}{You'd want to split the data yourself: [<-LINK->].} \\
\textit{Follow-up issue}: \textcolor{brown}{Can I use SplitTestAndTrain?}\\
\parbox[c]{12cm}{\textit{Solution for follow-up issue}: \textcolor{purple}{You could do split test and train on the batches and concatenate. If batchsize is the entire dataset, it should be fine, then yeah split test and train will work.}}
\end{tabular}\\
\hline

\begin{tabular}[c]{@{}l@{}}
{\LARGE \textbf{RICHA}}\\ 
\textit{Issue detection}: False\\
\textit{OQ solution detection}: \textcolor{blue}{You'd want to split the data yourself: [<-LINK->].}\\
\parbox[c]{12cm}{\textit{FQ solution detection}: Not really, unless you have the whole dataset in memory. You could go through the iterator and randomly do split test train and save the results.}
\end{tabular}\\
\hline
\end{tabular}}
\caption{Bad cases of our RICHA.}
\vspace{-0.5cm}

\label{tab:bad_cases}
\end{table}

==> tab/empirical_ablation.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[htbp]
 \resizebox{\columnwidth}{!}{
\begin{tabular}{|l|}
\hline
\begin{tabular}[c]{@{}l@{}}
{\LARGE \textbf{Raw Dialog}}\\ 
\parbox[c]{12cm}{\textcolor{red}{A: I'm training a DNN+CNN model. The F1 score is around 50. But there are some warnings that some classes are never predicted. Shall I create a dataset which is balanced for 5 types?}}\\
B: What do you mean "DNN+CNN " model? \\ 
\parbox[c]{12cm}{\textcolor{blue}{B: If you trained a conv net say that in plain English :D. Beyond that yes, minibatches should always be balanced.}}\\
\parbox[c]{12cm}{\textcolor{blue}{B: If you have a minibatch it should ideally be as close to representative of your whole population as possible, since the intuition for minibatch learning comes from statistics.}}\\
A: I mean danse Layer+CNN. I used wrong word, I guess.... \\
\parbox[c]{12cm}{B: The reason I ask about your model, is because batch size largely depends on dimensions of the data and kind of problem as well as number of labels. Then say "conv net" :D}\\ 
\parbox[c]{12cm}{\textcolor{blue}{B: The main thing it had going for it was the catalyst compiler for Tensorflow ops, which hasn't seemed a commit since August.}}\\
B: We also support configuring everything from a spark job.\\ 
B: Tensor frames for their JNI support used JavaCPP (which we maintain). \\ 
A: Nice! Thank you!\end{tabular}\\
\hline

\begin{tabular}[c]{@{}l@{}}
{\LARGE \textbf{Solution}}\\ 
\parbox[c]{12cm}{\textcolor{blue}{If you trained a conv net say that in plain English. Beyond that yes, minibatches should always be balanced. If you have a minibatch it should ideally be as close to representative of your whole population as possible, since the intuition for minibatch learning comes from statistics. The main thing it had going for it was the catalyst compiler for Tensorflow ops, which hasn't seemed a commit since August.}}\\
\end{tabular}\\
\hline

\begin{tabular}[c]{@{}l@{}}
{\LARGE \textbf{RICHA}}\\ 
\parbox[c]{12cm}{\textcolor{blue}{If you trained a conv net say that in plain English. Beyond that yes, minibatches should always be balanced. If you have a minibatch it should ideally be as close to representative of your whole population as possible, since the intuition for minibatch learning comes from statistics. The main thing it had going for it was the catalyst compiler for Tensorflow ops, which hasn't seemed a commit since August.} Tensor frames for their JNI support used JavaCPP (which we maintain).}\\
\end{tabular}\\
\hline

\begin{tabular}[c]{@{}l@{}}
{\LARGE \textbf{RICHA-LocalAttn}}\\ 
\parbox[c]{12cm}{What do you mean "DNN+CNN " model? \textcolor{blue}{If you trained a conv net say that in plain English. Beyond that yes, minibatches should always be balanced.} I mean danse Layer+CNN. I used wrong word, I guess... The reason I ask about your model, is because batch size largely depends on dimensions of the data and kind of problem as well as number of labels. Then say "conv net". Nice! Thank you!}\\
\end{tabular}\\
\hline

\begin{tabular}[c]{@{}l@{}}
{\LARGE \textbf{RICHA-Heu}}\\ 
\parbox[c]{12cm}{What do you mean "DNN+CNN " model? \textcolor{blue}{If you trained a conv net say that in plain English. If you have a minibatch it should ideally be as close to representative of your whole population as possible, since the intuition for minibatch learning comes from statistics. The main thing it had going for it was the catalyst compiler for Tensorflow ops, which hasn't seemed a commit since August.}}\\
\end{tabular}\\ \hline

\begin{tabular}[c]{@{}l@{}}
{\LARGE \textbf{RICHA-CNN}}\\
\parbox[c]{12cm}{What do you mean "DNN+CNN" model? \textcolor{blue}{If you trained a conv net say that in plain English. The main thing it had going for it was the catalyst compiler for Tensorflow ops, which hasn't seemed a commit since August.}}\\
\end{tabular}\\ \hline
\end{tabular}}
\caption{Test example of component analysis in solution prediction (DL4j).}
\vspace{-0.5cm}

\label{tab:example_ablation}
\end{table}

==> tab/empirical_baseline.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \vspace{-0.2cm}
\begin{table}[htbp]
\caption{Test example.}
\vspace{-0.2cm}
 \resizebox{\columnwidth}{!}{
\begin{tabular}{|l|}
\hline
\begin{tabular}[c]{@{}l@{}}
{\\\normalsize \textbf{Dialog}}\\ 
\parbox[c]{8.5cm}{\textcolor{purple}{($u_h$)A: I'm training a DNN+CNN model. The F1 score is around 50. But there are some warnings that some classes are never predicted. Shall I create a dataset which is balanced for five types?}}\\
($u_{b1}$)B: What do you mean ``DNN+CNN" model :( ?\\ 
\parbox[c]{8.5cm}{\textcolor{blue}{($u_{b2}$)B: Beyond trained on conv yes, minibatches should always be balanced.}}\\
\parbox[c]{8.5cm}{\textcolor{blue}{($u_{b3}$)B: If minibatch it should ideally be as close to representative of your whole population as possible.}}\\
($u_{b4}$)A: I mean danse Layer+CNN. I used wrong word, I guess.... \\
\parbox[c]{8.5cm}{($u_{b5}$)B: The reason why I ask is because batchsize largely depends on data dimension.}\\ 
\parbox[c]{8.5cm}{\textcolor{blue}{($u_{b6}$)B: The main thing it had going for it was the catalyst compiler for Tensorflow ops.}}\\
% ($u_7$)B: We also support configuring everything from a spark job.\\ 
% ($u_8$)B: Tensor frames for their JNI support used JavaCPP.  \\
{($u_{b7}$)A: Nice! Thank you!}\\
\end{tabular} \\ 
\hline

\begin{tabular}[c]{@{}l@{}}
{\\\normalsize \textbf{{\tool}}}\\\parbox[c]{8.5cm}{\textcolor{blue}{Beyond trained on conv yes, minibatches should always be balanced. If minibatch it should ideally be as close to representative of your whole population as possible. The main thing it had going for it was the catalyst compiler for Tensorflow ops.}} \\\end{tabular}\\ 
\hline

\begin{tabular}[c]{@{}l@{}}
{\\\normalsize \textbf{NB}
% \textbf{{\tool}-LocalAttn}
}\\\parbox[c]{8.5cm}{What do you mean ``DNN+CNN" model? \textcolor{blue}{Beyond trained on conv yes, minibatches should always be balanced.}}\\ \end{tabular}\\ \hline

\begin{tabular}[c]{@{}l@{}}
{\\\normalsize \textbf{RF}}\\\parbox[c]{8.5cm}{What do you mean ``DNN+CNN" model? \textcolor{blue}{Beyond trained on conv yes, minibatches should always be balanced.} I mean danse Layer+CNN. I used wrong word, I guess.}\\
\end{tabular}\\ \hline

\begin{tabular}[c]{@{}l@{}}
{\\\normalsize \textbf{GDBT}}\\\parbox[c]{8.5cm}{What do you mean ``DNN+CNN" model? \textcolor{blue}{Beyond trained on conv yes, minibatches should always be balanced.} I mean danse Layer+CNN, I used wrong word, I guess. The reason why I ask is because batchsize largely depends on data dimension. 
\textcolor{blue}{The main thing it had going for it was the catalyst compiler for Tensorflow ops.}}\\
\end{tabular}\\ \hline

\begin{tabular}[c]{@{}l@{}}
{\\\normalsize \textbf{UIT}
% \textbf{{\tool}-Heu}, \textbf{{\tool}-CNN}
}\\\parbox[c]{8.5cm}{\textcolor{blue}{Beyond trained on conv yes, minibatches should always be balanced. The main thing it had going for it was the catalyst compiler for Tensorflow ops.} Nice! Thank you!}\\
\end{tabular}\\ \hline

\begin{tabular}[c]{@{}l@{}}
{\\\normalsize \textbf{CNC\_SP}}\\\parbox[c]{8.5cm}{\textcolor{blue}{Beyond trained on conv yes, minibatches should always be balanced. If minibatch it should ideally be as close to representative of your whole population as possible.}}\\
\end{tabular}\\ \hline

\begin{tabular}[c]{@{}l@{}}
{\\\normalsize \textbf{DECA\_SP}}\\\textit{(Empty)}\\
\end{tabular}\\ \hline

% 后面这三个是消融实验的
% \begin{tabular}[c]{@{}l@{}}
% {\normalsize \textbf{{\tool}-LocalAttn}}\\ 
% \parbox[c]{8.5cm}{What do you mean "DNN+CNN " model? \textcolor{blue}{If you trained a conv net say that in plain English. Beyond that yes, minibatches should always be balanced.} I mean danse Layer+CNN. I used wrong word, I guess... The reason I ask about your model, is because batch size largely depends on dimensions of the data and kind of problem as well as number of labels. Then say "conv net". Nice! Thank you!}\\
% \end{tabular}\\
% \hline

% \begin{tabular}[c]{@{}l@{}}
% {\normalsize \textbf{{\tool}-Heu}}\\ 
% \parbox[c]{8.5cm}{What do you mean "DNN+CNN " model? \textcolor{blue}{If you trained a conv net say that in plain English. If minibatch it should ideally be as close to representative of your whole population as possible. The main thing it had going for it was the catalyst compiler for Tensorflow ops.}}\\
% \end{tabular}\\ \hline

% \begin{tabular}[c]{@{}l@{}}
% {\normalsize \textbf{{\tool}-CNN}}\\
% \parbox[c]{8.5cm}{What do you mean "DNN+CNN" model? \textcolor{blue}{If you trained a conv net say that in plain English. The main thing it had going for it was the catalyst compiler for Tensorflow ops.}}\\
% \end{tabular}\\ \hline
% \vspace{-0.2cm}
\end{tabular}}

\label{tab:example_baseline}
\end{table}

==> tab/heuristic_features.tex <==
% \linespread{1.5}
\begin{table*}[htbp]
\centering
 \resizebox{0.9\textwidth}{!}{
\begin{tabular}{|c|c|m{5.9cm}|c|c|c|}
\hline
\multirow{2}{*}{{\textbf{Feature Type}}} & \multirow{2}{*}{{ \textbf{Feature Name}}} & \multicolumn{4}{c|}{{\textbf{Feature Properties}}} \\
\cline{3-6} & & \multicolumn{1}{c|}{{ \textbf{Description}}} & \textbf{{ Data Type}} & \textbf{{ Data Field}}& \textbf{{ Example}} \\
\hline
\multirow{5}{*}{Keywords (12)}
& 5W1H & Occurrence of 5W1H interrogatives. & VECTOR & \{what, why, when, who, which, how\} & \{0,1,1,0,0,1\} \\ 
\cline{2-6} 
& Punctuation & Occurrence of question and exclamation. & VECTOR & \{question-mark, exclamation-mark\} & \{1, 0\}  \\ 
\cline{2-6} 
& Greeting & Occurrence of various greeting words. & BOOLEAN & True/False & 0 \\ 
\cline{2-6} 
& Disapproval & Occurrence of disapproval words. & BOOLEAN & True/False & 1 \\ 
\cline{2-6} 
& Repetition & Utterance may have similar/same expression. & VECTOR & \{simi-, same\} & \{0, 1\} \\ 
\hline
\multirow{5}{*}{Structure (5)}
& Token-length & Count of tokens in utterance. & DIGITAL & $[1, +\infty)$ & 25  \\ 
\cline{2-6} 
& Token-length (unique) & Count of unique tokens in utterance. & DIGITAL & $[1, +\infty)$ & 18  \\ 
\cline{2-6} 
& Token-length (stemmed) & Count of stemmed tokens in utterance. & DIGITAL & $[1, +\infty)$ & 10 \\ 
\cline{2-6} 
& Absolute position & Absolute position of utterance in dialog. & DIGITAL & $[1, +\infty)$ & 2  \\ 
\cline{2-6} 
& Relative position & Relative position of utterance in dialog. & DECIMAL & $[0, 1]$ & 0.20 \\ 
\hline
\multirow{2}{*}{Content (2)}
& TF-IDF simi. (head) & TF-IDF similarity between dialog head and the whole documentation of chat logs. & DECIMAL & $[0, 1]$ & 0.33  \\ 
\cline{2-6} 
& TF-IDF simi. (body) & TF-IDF similarity between utterance and the whole documentation of chat logs. & DECIMAL & $[0, 1]$ & 0.42   \\ 
\hline
\multirow{3}{*}{Sentiment (9)}
& Sentiment score & Polarity sentiment of NLTK analyzer. & VECTOR & \{positive, intermediate, negative\} & \{0.74, 0.31, 0.15\} \\ 
\cline{2-6} 
& Sentiment words & Count of \{pos., int., neg.\} sentiment words. & VECTOR & \{positive, intermediate, negative\} & \{4, 5, 1\} \\ 
\cline{2-6} 
& Emojis and acronyms & Count of \{pos., int., neg.\} emojis and acronyms. & VECTOR & \{positive, intermediate, negative\} & \{4, 1, 0\} \\ 
\hline
Role (1)
& Dialog initiator & Whether the speaker is the dialog initiator. & BOOLEAN & True/False & 1  \\
\hline
\end{tabular}}
\caption{The features in Heuristic Attribute Extractor.}
\vspace{-0.5cm}

\label{tab:heurustics}
\end{table*}

==> tab/practical.tex <==
\begin{table*}[htbp]
\caption{{\tool} in practice.}
\vspace{-0.2cm}
\centering
 \resizebox{0.9\textwidth}{!}{
\begin{tabular}{|c|c|c|c|m{6cm}|m{10cm}|c|}
\hline
\textbf{ID} & \textbf{Community} & \textbf{QID} & \textbf{Creation Time} & \multicolumn{1}{c|}{\textbf{Queried Issue}} & \multicolumn{1}{c|}{\textbf{{\tool}'s solution}} & \textbf{{\tool}'s contribution}  \\
\hline
1 & Materialize & 59282213 & 2019-12-1 & React Warning non-passive event listener to a scroll-blocking `touchstart'. & Check the fork for details on how to fix: https://github.com/materializecss/ materialize/issues/20 & Potential (1/2) \\
\hline
2 & Springboot & 66378380 & 2021-02-26 & Spring Boot 2.4.3 - Actuator /startup endpoint not found & Maybe you are using BootstrapApplicationListener which build the application context again but ignores the previous applicationStartup, so it sets the default, this is a bug in spring-cloud-context:3.0.0 & Commented (1/2)\\
\hline
3 & Springboot & 48915821  &  2018-03-12 & Application Fails to start with Springboot RC2 & You need to use Spring Cloud Finchley snapshots with RC2 & Potential (1/5)\\
\hline
4 & Springboot & 57543742 & 2019-08-18 &
When I start a microservice, SpringApplicationBuilder throw error & Maybe you have a mixed versions of spring boot jars & Potential (1/1)\\
\hline
5 & WebPack & 66868053 & 2020-04-30 & How to resolve this loader issue in react & If webpack runs tsc (the Typescript compiler) and complains about a .d.ts, that's weird. If Webpack says "I don't have a loader defined for .d.ts files", that means something tries to require a .d.ts and should never happen. & Potential (1/1)\\
% I've had this problem when people have a
% broad Context defined, either via require.context(/too-many-files.*\.ts/), or
% require("/some/path/" + fileName). Webpack will try to statically analyze the
% latter statement, and treat (more or less) as
% require.context(/\/some\/path\/.*/). Either way you wind up with it grabbing
% .d.ts files when it shouldn't. If you can fix the require / require.context so it
% excludes the typings do that If you can't add a rule like \{test: /\ d\ ts\$/ use
\hline
6 & WebPack & 66868545 & 2021-01-07 & Errors when transpiling to es5 using webpack 4 and babel &
% Did you try to hardcoded it to 44 instead of using babel_chrome_level? 
In Chrome devtools, you might be able to get it to pretty-print the minified Dojo sources to better identify exactly which feature it's tripping over. The better fix for this is to find whatever numbskull in your organization has you stuck on a FIVE YEAR OLD version of browsers and smack them til they stop. & Potential (1/1)\\
% Also it looks like you're explicitly excluding dojo from your Babel transform. I
% don't know much about Dojo -- I guess they made a totally new "modern"
% version at some point? -- but maybe you can pin to an older version of it that
% officially supports your version of Chrome?
\hline
7 & WebPack & 63620416 & 2020-08-27 &
Webpack imports all the unused exports into the bundle &
You may need to setup sideEffects in your package.json. https://webpack.js.org/guides/tree-shaking/ & Potential (1/1)\\
\hline
8 & WebPack & 66383230 & 2021-02-26 &
Couldn't find a style target which appears after SSR with React implementation. How to fix? &
I think you cannot use style-loader server side. Find the loader like this: https://github.com/codebandits/react-app-rewire-css-modules/blob/master/ index.js just use style-loader instead, and remove it.. or switch to razzle &
Potential (1/1)\\
\hline
\end{tabular}}
\vspace{-0.5cm}

\label{tab:practical}
\end{table*}

==> tab/rawset.tex <==
\begin{table}[htbp]
 \resizebox{\columnwidth}{!}{
\begin{tabular}{c|c|p{2.4cm}<{\centering}|c|c|c|c|c|c}
\toprule
\multirow{2}{*}{Id}&\multirow{2}{*}{Project} & \multirow{2}{*}{Domain} & \multicolumn{3}{c|}{Entire Population} & \multicolumn{3}{c}{Sample Population} \\
\cline{4-9}
& & & PA & Dial. & Utter.& SP & SD & SU \\ \hline
$P_1$& Angular          & Frontend Framework         & 22,467                 & 79,619            & 695,183              & 125                       & 97                       & 778                         \\ \hline
$P_2$& Appium          & Mobile                     & 3,979                  & 4,906             & 29,039               & 73                                      & 87                       & 724                         \\ \hline
$P_3$&Dl4j            & Data Science               & 8,310                  & 27,256            & 252,846              & 93                       & 100                       & 1,130                         \\ \hline
$P_4$&Docker           & DevOps                     & 8,810                  & 3,954             & 22,367               & 74               & 90                       & 1,126                         \\ \hline
$P_5$&Ethereum       & Blockchain Platform & 16,154                 & 17,298            & 91,028               & 116                       & 96                       & 516                         \\ \hline
$P_6$&Gitter         & Collabration Platform      & 9,260                  & 7,452             & 34,147               & 87                       & 86                       & 515                         \\ \hline
$P_7$&Typescript       & Programming Language                   & 8,318                  & 18,812            & 196,513              & 110              & 95                       & 1,700                         \\ \hline
$P_8$&Nodejs          & Web-App Framework  & 18,118                 & 13,981            & 81,771               & 144                       & 98                       & 737                         \\ \hline
\multicolumn{3}{c|}{\textit{Total}}          & \textit{95,416}        & \textit{173,278}  & \textit{1,402,894}    & \textit{822}             & \textit{749}             & \textit{7,226}               \\ \bottomrule
\end{tabular}
}
\caption{The characteristics of selected projects. 
%{\it Id} represents the serial number of projects, which identify the project name in follow-up sections. {\it Domain} represents the category which projects belong to. 
{\it PA} and {\it SP} represent the number of participants in the entire population and the representative sample dataset respectively. {\it Dial.} and {\it SD} represent the number of dialogues, {\it Utter.} and {\it SU} represent the number of utterances respectively.}
\label{project_prepration}
\end{table}

==> todo.tex <==
% citation 前面有个空格
% pos neg 计算 
% Table I, IV， V 字放大些
% 图、表位置合适且美观
%  {\website}  {XXX}
%  {\numPair}  {30K}
% {\numPairExp}  {21K}% 33-9
% percentage performance
% check 33K 24K
%live chat->live chats
% 所有Figure X 改成 Fig. X
% grammarly
% window-size to local window
% issue and solution models -> issue model and solution model
% 确认DECA 规则数量：6,51
% fix table VI
download pdf, make sure each number is correct
% 排版、图表位置等
% [1-9] 要用单词，3->three
% proof reading


website:  26 questions, 33K, code
